xNose: A Test Smell Detector for C#

Test smells, similar to code smells, can negatively impact both the test code and the production code being tested. Despite extensive research on test smells in languages like Java, Scala, and Python, automated tools for detecting test smells in C# are lacking. This paper aims to bridge this gap by extending the study of test smells to C#, and developing a tool (xNose) to identify test smells in this language and analyze their distribution across projects. We identified 16 test smells from prior studies that were language-independent and had equivalent features in C# and evaluated xNose, achieving a precision score of 96.97% and a recall score of 96.03%. In addition, we conducted an empirical study to determine the prevalence of test smells in xUnit-based C# projects. This analysis sheds light on the frequency and distribution of test smells, deepening our understanding of their impact on C# projects and test suites. The development of xNose and our analysis of test smells in C# code aim to assist developers in maintaining code quality by addressing potential issues early in the development process.

==> references.tex <==
@INPROCEEDINGS{In1,
  author={Saca, Mauricio A.},
  booktitle={2017 IEEE 37th Central America and Panama Convention (CONCAPAN XXXVII)}, 
  title={Refactoring improving the design of existing code}, 
  year={2017},
  volume={},
  number={},
  pages={1-3},
  doi={10.1109/CONCAPAN.2017.8278488}}

  
  @article{In2,
  title={Comparing and experimenting machine learning techniques for code smell detection},
  author={Francesca Arcelli Fontana and Mika M{\"a}ntyl{\"a} and Marco Zanoni and Alessandro Marino},
  journal={Empirical Software Engineering},
  year={2016},
  volume={21},
  pages={1143-1191}
}
@article{In3,
  title={An empirical study of the bad smells and class error probability in the post-release object-oriented system evolution},
  author={Wei Li and Raed Shatnawi},
  journal={J. Syst. Softw.},
  year={2007},
  volume={80},
  pages={1120-1128}
}
@article{In4,
  title={An Empirical Study of Design Degradation: How Software Projects Get Worse over Time},
  author={Iftekhar Ahmed and Umme Ayda Mannan and Rahul Gopinath and Carlos Jensen},
  journal={2015 ACM/IEEE International Symposium on Empirical Software Engineering and Measurement (ESEM)},
  year={2015},
  pages={1-10}
}
@article{In5,
  title={The evolution and impact of code smells: A case study of two open source systems},
  author={Steffen M. Olbrich and Daniela Soares Cruzes and Victor R. Basili and Nico Zazworka},
  journal={2009 3rd International Symposium on Empirical Software Engineering and Measurement},
  year={2009},
  pages={390-400}
}
@article{In6,
  title={Some Code Smells Have a Significant but Small Effect on Faults},
  author={Tracy Hall and Min Zhang and David Bowes and Yi Sun},
  journal={ACM Trans. Softw. Eng. Methodol.},
  year={2014},
  volume={23},
  pages={33:1-33:39}
}
@inproceedings{In7,
  title={Investigating the impact of design debt on software quality},
  author={Nico Zazworka and Michele A. Shaw and Forrest Shull and Carolyn Budinger Seaman},
  booktitle={MTD '11},
  year={2011}
}
@article{In8,
  title={When and Why Your Code Starts to Smell Bad (and Whether the Smells Go Away)},
  author={Michele Tufano and Fabio Palomba and Gabriele Bavota and Rocco Oliveto and Massimiliano Di Penta and Andrea De Lucia and Denys Poshyvanyk},
  journal={IEEE Transactions on Software Engineering},
  year={2015},
  volume={43},
  pages={1063-1088}
}
@article{In9,
  title={Refactoring test code},
  author={Arie van Deursen and Leon Moonen and Armand van den Bergh and G. Kok},
  journal={Report - Software engineering},
  year={2001},
  pages={1-6}
}
@article{In10,
  title={An empirical analysis of the distribution of unit test smells and their impact on software maintenance},
  author={Gabriele Bavota and Abdallah Qusef and Rocco Oliveto and Andrea De Lucia and David W. Binkley},
  journal={2012 28th IEEE International Conference on Software Maintenance (ICSM)},
  year={2012},
  pages={56-65}
}
@article{In11,
  title={On the Relation of Test Smells to Software Code Quality},
  author={Davide Spadini and Fabio Palomba and Andy Zaidman and Magiel Bruntink and Alberto Bacchelli},
  journal={2018 IEEE International Conference on Software Maintenance and Evolution (ICSME)},
  year={2018},
  pages={1-12}
}
@article{In13,
  title={An Empirical Study on the Evolution of Test Smell},
  author={Dong Jae Kim},
  journal={2020 IEEE/ACM 42nd International Conference on Software Engineering: Companion Proceedings (ICSE-Companion)},
  year={2020},
  pages={149-151}
}
@article{In12,
  title={Are test smells really harmful? An empirical study},
  author={Gabriele Bavota and Abdallah Qusef and Rocco Oliveto and Andrea De Lucia and David W. Binkley},
  journal={Empirical Software Engineering},
  year={2014},
  volume={20},
  pages={1052 - 1094}
}
@article{In14,
  title={Automated Detection of Test Fixture Strategies and Smells},
  author={Michaela Greiler and Arie van Deursen and Margaret-Anne D. Storey},
  journal={2013 IEEE Sixth International Conference on Software Testing, Verification and Validation},
  year={2013},
  pages={322-331}
}
@inproceedings{In15,
  title={Assessing diffusion and perception of test smells in scala projects},
  author={Jonas De Bleser and Dario Di Nucci and Coen De Roover},
  booktitle={IEEE Working Conference on Mining Software Repositories},
  year={2019}
}
@article{In16,
  title={TEMPY: Test Smell Detector for Python},
  author={Daniel Fernandes and Ivan Machado and Rita Suzana Pitangueira Maciel},
  journal={Proceedings of the XXXVI Brazilian Symposium on Software Engineering},
  year={2022}
}
@article{In17,
  title={PyNose: A Test Smell Detector For Python},
  author={Tongjie Wang and Yaroslav Golubev and Oleg Smirnov and Jiawei Li and Timofey Bryksin and Iftekhar Ahmed},
  journal={2021 36th IEEE/ACM International Conference on Automated Software Engineering (ASE)},
  year={2021},
  pages={593-605}
}
@misc{In18,
  author = {Lionel Sujay Vailshery},
  title = {Worldwide Developer Survey: Most Used Programming Languages 2021},
  howpublished = {\url{https://www.statista.com/statistics/793628/worldwide-developer-survey-most-used-languages/}},
  year = {2021},
  note = {Accessed: February 20, 2023}
}
@unknown{In19,
author = {Aljedaani, Wajdi and Peruma, Anthony and Aljohani, Ahmed and Alotaibi, Mazen and Mkaouer, Mohamed Wiem and Ouni, Ali and Newman, Christian and Ghallab, Abdullatif and Ludi, Stephanie},
year = {2021},
month = {04},
pages = {},
title = {Test Smell Detection Tools: A Systematic Mapping Study}
}
@book{R20,
  title={The Hitchhiker's guide to Python: best practices for development},
  author={Reitz, Kenneth and Schlusser, Tanya},
  year={2016},
  publisher={" O'Reilly Media, Inc."}
}
@inproceedings{R21,
  title={xUnit Test Patterns: Refactoring Test Code},
  author={Gerard Meszaros},
  year={2007}
}

@INPROCEEDINGS{R22,
  author={Van Rompaey, Bart and Du Bois, Bart and Demeyer, Serge},
  booktitle={2006 22nd IEEE International Conference on Software Maintenance}, 
  title={Characterizing the Relative Significance of a Test Smell}, 
  year={2006},
  volume={},
  number={},
  pages={391-400},
  doi={10.1109/ICSM.2006.18}}

  @inproceedings{R23,
  title={Testq: Exploring structural and maintenance characteristics of unit test suites},
  author={Breugelmans, Manuel and Van Rompaey, Bart},
  booktitle={WASDeTT-1: 1st International Workshop on Advanced Software Development Tools and Techniques},
  year={2008},
  organization={Citeseer}
}
@inproceedings{R24,
  title={Socrates: Scala radar for test smells},
  author={De Bleser, Jonas and Di Nucci, Dario and De Roover, Coen},
  booktitle={Proceedings of the Tenth ACM SIGPLAN Symposium on Scala},
  pages={22--26},
  year={2019}
}
@article{R25,
  title={On the distribution of test smells in open source android applications: An exploratory study},
  author={Peruma, Anthony and Almalki, Khalid Saeed and Newman,  Christian D and Mkaouer, Mohamed Wiem and Ouni, Ali and Palomba, Fabio},
  year={2019}
}
@inproceedings{R26,
  title={On the influence of test smells on test coverage},
  author={Virg{\'\i}nio, T{\'a}ssio and Santana, Railana and Martins, Luana Almeida and Soares, Larissa Rocha and Costa, Heitor and Machado, Ivan},
  booktitle={Proceedings of the XXXIII Brazilian Symposium on Software Engineering},
  pages={467--471},
  year={2019}
}
@article{R27,
  title={On the detection of test smells: A metrics-based approach for general fixture and eager test},
  author={Van Rompaey, Bart and Du Bois, Bart and Demeyer, Serge and Rieger, Matthias},
  journal={IEEE Transactions on software engineering},
  volume={33},
  number={12},
  pages={800--817},
  year={2007},
  publisher={IEEE}
}
@inproceedings{R28,
  title={Automatic test smell detection using information retrieval techniques},
  author={Palomba, Fabio and Zaidman, Andy and De Lucia, Andrea},
  booktitle={2018 IEEE International Conference on Software Maintenance and Evolution (ICSME)},
  pages={311--322},
  year={2018},
  organization={IEEE}
}
@inproceedings{R29,
  title={Tsdetect: An open source test smells detection tool},
  author={Peruma, Anthony and Almalki, Khalid and Newman, Christian D and Mkaouer, Mohamed Wiem and Ouni, Ali and Palomba, Fabio},
  booktitle={Proceedings of the 28th ACM joint meeting on european software engineering conference and symposium on the foundations of software engineering},
  pages={1650--1654},
  year={2020}
}
@inproceedings{R30,
  title={Just-in-time test smell detection and refactoring: The darts project},
  author={Lambiase, Stefano and Cupito, Andrea and Pecorelli, Fabiano and De Lucia, Andrea and Palomba, Fabio},
  booktitle={Proceedings of the 28th international conference on program comprehension},
  pages={441--445},
  year={2020}
}
@inproceedings{R31,
  title={RAIDE: a tool for Assertion Roulette and Duplicate Assert identification and refactoring},
  author={Santana, Railana and Martins, Luana and Rocha, Larissa and Virg{\'\i}nio, T{\'a}ssio and Cruz, Adriana and Costa, Heitor and Machado, Ivan},
  booktitle={Proceedings of the XXXIV Brazilian Symposium on Software Engineering},
  pages={374--379},
  year={2020}
}
@inproceedings{R32,
  title={Jnose: Java test smell detector},
  author={Virg{\'\i}nio, T{\'a}ssio and Martins, Luana and Rocha, Larissa and Santana, Railana and Cruz, Adriana and Costa, Heitor and Machado, Ivan},
  booktitle={Proceedings of the XXXIV Brazilian Symposium on Software Engineering},
  pages={564--569},
  year={2020}
}
@misc{aspnetboilerplate,
  title={Aspnetboilerplate},
  howpublished={\url{https://github.com/aspnetboilerplate/aspnetboilerplate}},
  year={Accessed 2023-15-01}
}

@misc{nlog,
  title={NLog},
  howpublished={\url{https://github.com/NLog/NLog}},
  year={Accessed 2023-15-01}
}

@misc{c4sharp,
  title={C4Sharp},
  howpublished={\url{https://github.com/8T4/c4sharp}},
  year={Accessed 2023-15-01}
}

@misc{ocelot,
  title={Ocelot},
  howpublished={\url{https://github.com/ThreeMammals/Ocelot}},
  year={Accessed 2023-15-01}
}

@misc{skoruba,
  title={Skoruba.IdentityServer4.Admin},
  howpublished={\url{https://github.com/IdentityServer/IdentityServer4}},
  year={Accessed 2023-15-01}
}

@misc{scrutor,
  title={Scrutor},
  howpublished={\url{https://github.com/khellang/Scrutor}},
  year={Accessed 2023-15-01}
}

@misc{refit,
  title={Refit},
  howpublished={\url{https://github.com/reactiveui/refit}},
  year={Accessed 2023-15-01}
}

@misc{greendonut,
  title={GraphQl-Platform.GreenDonut},
  howpublished={\url{https://github.com/ChilliCream/graphql-platform}},
  year={Accessed 2023-15-01}
}

@misc{hotchocolatecaching,
  title={GraphQl-Platform.HotChocolate.Caching},
  howpublished={\url{https://github.com/ChilliCream/graphql-platform}},
  year={Accessed 2023-15-01}
}

@misc{hotchocolatecore,
  title={GraphQl-Platform.HotChocolate.Core},
  howpublished={\url{https://github.com/ChilliCream/graphql-platform}},
  year={Accessed 2023-15-01}
}

@misc{eshoponweb,
  title={eShopOnWeb},
  howpublished={\url{https://github.com/dotnet-architecture/eShopOnWeb}},
  year={Accessed 2023-15-01}
}
@inproceedings{M34,
  title={Guidelines for snowballing in systematic literature studies and a replication in software engineering},
  author={Wohlin, Claes},
  booktitle={Proceedings of the 18th international conference on evaluation and assessment in software engineering},
  pages={1--10},
  year={2014}
}
@book{M33,
  title={Evidence-based software engineering and systematic reviews},
  author={Kitchenham, Barbara Ann and Budgen, David and Brereton, Pearl},
  volume={4},
  year={2015},
  publisher={CRC press}
}
@misc{M35,
  title={Guidelines for performing systematic literature reviews in software engineering},
  author={Keele, Staffs and others},
  year={2007},
  publisher={Technical report, ver. 2.3 ebse technical report. ebse}
}
@inproceedings{M38,
  title={Exploring the benefits of utilizing conceptual information in test-to-code traceability},
  author={Kicsi, Andr{\'a}s and T{\'o}th, L{\'a}szl{\'o} and Vid{\'a}cs, L{\'a}szl{\'o}},
  booktitle={Proceedings of the 6th International Workshop on Realizing Artificial Intelligence Synergies in Software Engineering},
  pages={8--14},
  year={2018}
}
@inproceedings{M39,
  title={Testroutes: A manually curated method level dataset for test-to-code traceability},
  author={Kicsi, Andr{\'a}s and Vid{\'a}cs, L{\'a}szl{\'o} and Gyim{\'o}thy, Tibor},
  booktitle={Proceedings of the 17th International Conference on Mining Software Repositories},
  pages={593--597},
  year={2020}
}
@inproceedings{M40,
  title={Automatically identifying focal methods under test in unit test cases},
  author={Ghafari, Mohammad and Ghezzi, Carlo and Rubinov, Konstantin},
  booktitle={2015 IEEE 15th International Working Conference on Source Code Analysis and Manipulation (SCAM)},
  pages={61--70},
  year={2015},
  organization={IEEE}
}
@misc{xunitnet,
  title = {Documentation},
  author = {{xUnit.net}},
  howpublished = {Retrieved March 1, 2023, from \url{https://xunit.net/\#documentation}},
  year = {n.d.}
}

@misc{dotnet-corefx,
  title={Dotnet Corefx},
  howpublished={\url{https://github.com/939481896/dotnet-corefx/commit/1296bc8386a7283e319ddf723282f16651f9ea5f}},
  year={Accessed 2022-13-12}
}
@misc{nlog-commit,
  title={NLog},
  author={NLog},
  howpublished={\url{https://github.com/NLog/NLog/commit/151a106428df0058cc1a74c85d474bc89cc6bb6e}},
  year={Accessed 2022-15-11}
}
@misc{cyclometic,
  title={Cyclometic Complexity of Methods},
  author={Microsoft},
  howpublished={\url{https://learn.microsoft.com/en-us/visualstudio/code-quality/code-metrics-cyclomatic-complexity?view=vs-2022}},
  year={Accessed 2022-15-10}
}
@misc{vs,
  title={Visual Studio},
  howpublished={\url{https://visualstudio.microsoft.com/}},
  year={Accessed 2022-15-10}
}
@misc{roslyn,
  title={Roslyn Api},
  howpublished={\url{https://learn.microsoft.com/en-us/dotnet/csharp/roslyn-sdk/}},
  year={Accessed 2022-15-10}
}
 @misc{ndepend, title={Code diff since baseline}, url={https://www.ndepend.com/features/code-diff#BuildComparison}, journal={NDepend}, publisher={NDepend}, author={NDepend}} 

@misc{inppropriate-assertion,
  title = {Test Smell Catalog},
  url = {https://test-smell-catalog.readthedocs.io/en/latest/Issues%20in\%20test%20steps/Issues%20in%20assertions/Inappropriate%20Assertions.html},
  year = {Accessed on December 20, 2022}
}

@misc{emperical-dataset,
  title = {Dataset for Empirical Study},
  url = {https://anonymous.4open.science/r/xNose-4D3E/repoCollection.json},
  year = {Accessed on July 13, 2023}
}
